Variational Automatic Curriculum Learning for Sparse-Reward Cooperative Multi-Agent Problems

We introduce a curriculum learning algorithm, Variational Automatic Curriculum Learning (VACL), for solving challenging goal-conditioned cooperative multi-agent reinforcement learning problems. We motivate our paradigm through a variational perspective, where the learning objective can be decomposed into two terms: task learning on the current task distribution, and curriculum update to a new task distribution. Local optimization over the second term suggests that the curriculum should gradually expand the training tasks from easy to hard. Our VACL algorithm implements this variational paradigm with two practical components, task expansion and entity progression, which produces training curricula over both the task configurations as well as the number of entities in the task. Experiment results show that VACL solves a collection of sparse-reward problems with a large number of agents. Particularly, using a single desktop machine, VACL achieves 98% coverage rate with 100 agents in the simple-spread benchmark and reproduces the ramp-use behavior originally shown in OpenAI's hide-and-seek project. Our project website is at https://sites.google.com/view/vacl-neurips-2021.

==> 50related.tex <==
Curriculum learning~\cite{bengio2009curriculum} is a popular training paradigm for RL problems in various domains~\cite{narvekar2020curriculum}. 
We focus on goal-conditioned multi-agent cooperative problems and assume a paramterized task space. This is a common setting in the recent \underline{A}utomatic \underline{C}urriculum \underline{L}earning (ACL) literature~\cite{portelas2020automatic}. 
Some ACL works also consider a fixed set of tasks to solve~\cite{matiisen2019teacher}, which are typically referred to as multi-task learning~\cite{yang2020multitask}. 
The core idea in ACL literature is to discover tasks with moderate difficulty, i.e., neither too hard nor too easy, for the current policy and only use these tasks for training. 
This principle naturally emerges as a result of our variational inference paradigm.

A popular class of ACL methods learn a generative model over the task space with density concentrated on tasks with the desired difficulty. Popular model choices include VAE~\cite{Racaniere2020Automated}, GAN~\cite{florensa2018automatic,fang2021adaptive} and Gaussian mixture models~\cite{portelas2019teacher,jabri2019unsupervised,morad2021embodied}.
These methods can be viewed as a generic solution under our variational training objective by directly learning a new task proposal distribution from scratch whenever the policy is updated. However, when repeatedly learning a generative model may require extremely high sample complexity, which can be inefficient for problems with a low-dimensional task representation available (e.g., state-based tasks).

Another ACL framework is particle-based approach, which maintains a set of task samples that are easy to solve and gradually expands the set towards the entire space.
\citet{florensa2017reverse} and \citet{ivanovic2019barc} assume a fixed goal and generate training tasks with starting states increasingly far away from the goal; \citet{akkaya2019solving} and \citet{mehta2020active} consider a task space over simulator configurations and train from the easiest setting to the hardest setting for sim-to-real adaptation.  
These methods are conceptually similar to the \emph{task expansion} component in {\name}, which leverages stein variational inference for curriculum update. However, comparing with existing particle-based methods, our methods have major algorithmic innovations thanks to our variational paradigm. More discussions are presented in Sec.~\ref{sec:discuss}.
Besides, \citet{wang2019poet,wang2020enhanced} learn an individual policy paired with each task in the set for discovering diverse emergent behaviors while our work focuses on learning a single goal-conditioned policy for the entire task space; \citet{wohlke2020performance} propose to learn to more effectively expand the task set, which is complementary to our work. 
\reminder{AMIGo}


% Although these methods are general enough to capture arbitrarily high-dimensional task space (e.g., visual tasks) with an expressive function approximator, learning a generative model itself may require extremely high sample complexity, which can be inefficient for problems with a low-dimensional task representation available (e.g., most state-based tasks). A low-dimensional alternative is to use a particle-based approach, which maintains a set of task samples that are easy to solve and gradually expands the set towards the entire space.
% \citet{florensa2017reverse} and \citet{ivanovic2019barc} assume a fixed goal and generate training tasks with starting states increasingly far away from the goal; \citet{akkaya2019solving} and \citet{mehta2020active} consider a task space over simulator configurations and train from the easiest setting to the hardest setting for sim-to-real adaptation; \citet{wang2019poet,wang2020enhanced} learn an individual policy paired with each task in the set for discovering diverse emergent behaviors. 
% The \emph{task expansion} component in our method falls into this class of approaches. 
% Particularly, we assume each task can be represented by a starting state and a goal, and learn a single goal-conditioned policy to solve all possible tasks in a fixed physical environment. 
%Besides, \citet{wohlke2020performance} propose to learn to explore novel tasks for more effective set expansion, which is complementary to our work. 


A unique challenge in MARL is the additional complexity due to the large number of agents in the problem.
\citet{long2020evolutionary,wang2019largescale} propose \emph{population curriculum}, which trains entity-invariant policies over training tasks with a growing number of agents. 
\citet{feng2020solving} study the Sokoban game with a similar curriculum learning method over an increasing number of boxes in the game.
These methods tackle the same challenge as the \emph{entity progression} component in {\name} and can be viewed as a special case as our approach. 
There are also other works studying policy representation improvements for problems with massive agents~\cite{pmlr-v80-yang18d,NIPS2018_7956}, which are orthogonal to our focus. 

% Multi-agent problems bring additional complexities for single-agent ACL methods, particularly when the agent amount is large. %Note that the number of agents influences the dimension of input state to the policy.
% \citet{long2020evolutionary,wang2019largescale} propose \emph{population curriculum}, which trains entity-invariant policies from games with only a few agents first and then gradually increases the agent number to tackle problems with massive agents. 
% %Our \emph{entity curriculum} component inherits the population curriculum framework and additionally proposes a new mixed-switch technique to improve training when the number of agents grows. 
% There are also other works tackling tasks with a large number of agents via improved policy representation~\cite{pmlr-v80-yang18d,NIPS2018_7956}, which are orthogonal to our focus. 
% \citet{feng2020solving} study the Sokoban game, where the number of boxes is strongly related to the game difficulty, and propose to build a training curriculum over the box amount. 
% Our \emph{entity curriculum} component extends \emph{population curriculum} by unifying agents and objects (e.g., boxes) as entities of different types and representing the entity configuration as a discrete-valued multi-dimensional vector. A novel mixed-switch technique is also proposed to stabilize training when the number of entities grows. 

We consider cooperative tasks for the clear measurement of training progress.
Existing works also study autocurricula for competitive games~\citep{sukhbaatar2018intrinsic,leibo2019autocurricula,baker2020emergent}, which we leave as future work. 


==> pesudo.tex <==
\begin{algorithm}[bt!]
  \caption{Task Expansion Specific Functions}
  \label{algo:enhancements}

  % set funcion sample
  %\tcc{Sample a batch of training tasks}
  \SetKwFunction{Fsample}{\textbf{Sample}}
  \SetKwProg{Fn}{Def}{:}{}
  \Fn{\Fsample{$[\mathcal{M}^{e}_{sol}, \mathcal{M}^{e}_{act},\mathcal{M}^{e}_{nxt}]$, $B$}}
  {     
    $\mathcal{M}^{e}_{train}\leftarrow\textbf{Unif}(\mathcal{M}^{e}_{act}, B_{act})+\textbf{Unif}(\mathcal{M}^{e}_{nxt}, B_{nxt})$
    
        \tcc{\textbf{past sampling} from solved set}
        $\mathcal{M}^{e}_{train}\leftarrow\mathcal{M}^{e}_{train}+\textbf{Unif}(\mathcal{M}^{e}_{sol}, B_{sol})$
        
        \KwRet $\mathcal{M}^{e}_{train}$
  }
  
  % set function explore
  \SetKwFunction{Fexplore}{\textbf{Explore}}
  %\SetKwProg{Fn}{Def}{:}{}
  %\tcc{Explore nearby tasks from $\mathcal{M}^e_{train}$}
  \Fn{\Fexplore{$\mathcal{M}^{e}_{train}$,$\{\sigma_j\}$, $\sigma_{\min}$, $\sigma_{\max}$}}
  {
        
  
        \tcc{\textbf{$\sigma_{\max}$-selection}: only explore from newly solved tasks}
        $\mathcal{M}^e_{parent}\gets\{\phi_j:\phi_j \in M^e_{train}\land \sigma_j>\sigma_{\max}\}$
        
        \tcc{$\delta_{ns}$:  \textbf{novelty} threshold}
        $\delta_{ns}\gets \textrm{mean}(\{\textbf{Novelty}(\phi_j):\phi_j\in\mathcal{M}_{sol}^e\})$
        
        
        $\mathcal{M}^{e}_{nxt}\leftarrow \{\}$
        
        \While{$\|\mathcal{M}^{e}_{nxt}\| < B_{nxt}$}
        {
            $\phi_j\gets\textbf{Unif}(\mathcal{M}^e_{parent})$
            
            \tcc{$\alpha$: exploration step size}
            $\phi'\gets \phi_j+\alpha\cdot \textbf{Rand}(-1,1,\textbf{Sizeof}(\phi_j))$
            
            \tcp{\textbf{novelty search}}
            \If{$\textbf{\emph{Novelty}}(\phi')>\delta_{ns}$}
            {
            %\tcp{only keep novel samples}
            $\mathcal{M}^e_{nxt}\gets\mathcal{M}^e_{nxt}+\{\phi'\}$
            }
        }
        \KwRet $\mathcal{M}^{e}_{nxt}$
  }
  
  
  
  % set funcion Filter
  \SetKwFunction{Ffilter}{\textbf{Filter}}
  %\SetKwProg{Fn}{Def}{:}{}
  
  %\tcc{Update $\mathcal{M}^e_{act}$ with trained tasks}
  \Fn{\Ffilter{$\mathcal{M}^{e}_{act},\mathcal{M}^{e}_{train}$,$\{\sigma_j\}$,$\sigma_{\min}$,$\sigma_{\max}$}}
  {
       % select normal state 
       \tcc{\textbf{$\sigma_{\max}$-selection}: remove solved tasks from active set  $\mathcal{M}^e_{act}$}
       $\mathcal{M}^e_{act}\gets \mathcal{M}^e_{act}\setminus\{\phi_j:\phi_j\in\mathcal{M}^e_{train}\,\land\, \sigma_j >\sigma_{\max}\}$
       
       \tcc{$\mathcal{M}^e_{new}$: active training tasks}
       $\mathcal{M}^e_{new}\gets \{\phi_j: \sigma_{\min}\le \sigma_j \le \sigma_{\max}\}$
       
       % diversified buffer
       \tcc{\textbf{Diversified set}}
       $\mathcal{M}^e_{act}\gets\textbf{Diversify}(\mathcal{M}^e_{act}+\mathcal{M}^e_{new}, N_{act})$ \\
       \tcp{keep at most $N_{act}$ diverse tasks}
       
        \KwRet $\mathcal{M}^{e}_{act}$
  }
 \end{algorithm}
 
